Metabelianisations of finitely presented groups

In this article, I study some classes of finitely presented groups with the aim of finding out whether the maximal metabelian quotients of the members of these classes admit finite presentations. The considered classes include those of soluble groups, of one-relator or knot groups, and of Artin groups.

==> 10.Remainders.tex <==
%%
\section{Concluding remarks}
\label{sec:Concluding-remarks}
%%
%
Here are some brief comments 
on various aspects of the actual version of the paper.
\begin{itemize}

\item \emph{Introduction:}
Add acknowledgements

\item \emph{Section 3:}
To solve Problem 3.4 (on page 6) one should know more instances
where Theorem 3.3 is applicable, but not Theorem 3.1.

\item \emph{Section 4 (soluble groups):}
The title requires that the groups have no non-abelian free subgroups;
as examples,
I mention soluble groups and groups of PL-homeomorphisms.
Other groups are those of intermediate growth,
but I don't know whether it is appropriate to include such groups into my article.

\item \emph{Section 6 (knot groups):}
It is not yet clear to me
whether Illustration 6.2 deserves to be maintained in a final version.
The discussed group is a one-relator group 
with two generators and infinite cyclic abelianisation.
So one could include it in illustration 5.5 as a second example 
or as an example replacing the actual example.

\item \emph{Section 7:}
Theorem 7.1 holds for every Artin group.
In order to find out 
whether the $G = \Gamma/\Gamma''$ is finitely presentable 
it suffices thus to determine 
whether this top is polycyclic.
This verification may also be possible for groups
which are not covered by the results in Section 7.

A simple example of a group of this new type the is
\begin{equation}
\label{eq:Sticky-example}
\Gamma =
\langle a, a, c, d\mid
aba = bab, (bc)^2 = (cb)^2, cdc = dcd, (da)^3 = (ad)^3 \rangle.
\end{equation}
The abelianisation of $\Gamma$ is free abelian of rank 2
and so one should be able to study
\[
H_1(\Gamma', \Z) \iso H_1(\Gamma, \Z{\Gamma_{\ab}})
\]
with the help of the given presentation 
and the partial resolution going back to Lyndon \cite{Lyn50}
(\cf formula \eqref{eq:Lyndons-resolution}).

\item \emph{Section 7:} According to \cite{RhRo06} the derived groups of most of the irreducible Artin groups of finite type are \emph{perfect},
those of type $A_\ell$ for $\ell \geq 4$,
of type $B_\ell $ for $\ell \geq 5$, 
of type $D_\ell$ for $\ell \geq 5$, 
of type $E_6$, $E_7$, and $E_8$, 
and those of types $H_3$ and $H_4$.
Find a new proof of this fact, 
by establishing directly that the derived groups of the groups of type $A_4$ and $B_5$ are perfect, 
and then using the idea of the proof of Theorem
\ref{thm:Groups-with-infinite-cyclic-abelianisation}.
(19/08/2018(It seems that I can prove every claim;
the techniques include Presentations (for H3), homological algebra and 
Theorem
\ref{thm:Groups-with-infinite-cyclic-abelianisation}.
\end{itemize}






==> Definitions.tex <==
%
\makeatletter
%
%
\def\ab{\mathop{\operator@font ab}\nolimits}
\def\ad{\mathop{\operator@font ad}\nolimits}
\def\Ad{\mathop{\operator@font Ad}\nolimits}
\def\add{\mathop{\operator@font add}\nolimits}
\def\Aff{\mathop{\operator@font Aff}\nolimits}
\def\AG{\mathop{\operator@font AG}\nolimits}
\def\Alt{\mathop{\operator@font Alt}\nolimits}
\def\Ann{\mathop{\operator@font Ann}\nolimits}
\def\Aut {\mathop{\operator@font Aut  }\nolimits}
%
\def\BPL {\mathop{\operator@font BPL  }\nolimits}
%
\def\can {\mathop{\operator@font can  }\nolimits}
\def\card {\mathop{\operator@font card  }\nolimits}
\def\cd{\mathop{\operator@font cd}\nolimits}
\def\ch{\mathop{\operator@font char}\nolimits}
\DeclareMathOperator{\Cohom}{H} 

\def\coker {\mathop{\operator@font coker }\nolimits}
\def\colim {\mathop{\operator@font colim }\nolimits}
\def\core {\mathop{\operator@font core  }\nolimits}

\def\defi {\mathop{\operator@font def }\nolimits}
\def\Der {\mathop{\operator@font Der }\nolimits}
\def\diag {\mathop{\operator@font diag }\nolimits}
\def\dis {\mathop{\operator@font dis }\nolimits}
\def\dom {\mathop{\operator@font dom }\nolimits}
\def\Dr {\mathop{\operator@font Dr }\nolimits}
\def\edg {\mathop{\operator@font edg  }\nolimits}

\def\Eu {\mathop{\operator@font E  }\nolimits}
\def\End {\mathop{\operator@font End  }\nolimits}
\def\Ext {\mathop{\operator@font Ext }\nolimits}
\def\even {\mathop{\operator@font even  }\nolimits} 

\def\face {\mathop{\operator@font face }\nolimits}
\def\Fit {\mathop{\operator@font Fit }\nolimits}
\def\FP {\mathop{\operator@font FP }\nolimits}
\def\Frat {\mathop{\operator@font Frat  }\nolimits}

\def\gp{\mathop{\operator@font gp  }\nolimits}
\def\gcd{\mathop{\operator@font gcd  }\nolimits}
\def\GL{\mathop{\operator@font GL }\nolimits}

\def\Hom {\mathop{\operator@font Hom }\nolimits}
%
\def\id{\mathbbm{1}}
\def\im{\mathop{\operator@font im }\nolimits}
\def\Inn {\mathop{\operator@font Inn  }\nolimits}
\def\Iso{\mathop{\operator@font Iso}\nolimits}
%
%
\def\md {\mathop{\operator@font md  }\nolimits}
\def\mod{\mathop{\operator@font mod }\nolimits}
\newcommand{\norm}[1]{\| #1\|}

\def\odd {\mathop{\operator@font odd  }\nolimits} 

\def\PL {\mathop{\operator@font PL  }\nolimits} 
\DeclareMathOperator{\Perm}{Perm} 

\def\res {\mathop{\operator@font res }\nolimits} 
\def\rk {\mathop{\operator@font rk  }\nolimits} 

\def\sd {\mathop{\operator@font sd  }\nolimits}
\def\sgp {\mathop{\operator@font sgp  }\nolimits}
\def\sign {\mathop{\operator@font sign  }\nolimits}
\def\SL{\mathop{\operator@font SL }\nolimits}
\def\SO{\mathop{\operator@font SOL }\nolimits}
\def\Sol{\mathop{\operator@font Sol }\nolimits}
%
\def\myspan {\mathop{\operator@font span}\nolimits} 
\def\stab {\mathop{\operator@font stab  }\nolimits}
\def\supp {\mathop{\operator@font supp  }\nolimits}
\def\SUPP {\mathop{\operator@font SUPP  }\nolimits}
\def\sym {\mathop{\operator@font sym  }\nolimits}
\def\Sym {\mathop{\operator@font Sym  }\nolimits}
\def\Sp{\mathop{\operator@font Sp }\nolimits}

\def\Tor {\mathop{\operator@font Tor  }\nolimits}
\def\TPL {\mathop{\operator@font TPL  }\nolimits}

\def\Val {\mathop{\operator@font Val  }\nolimits}
\def\ver {\mathop{\operator@font ver  }\nolimits} 
%%
%%
\def\B{\mathbb{B}} 
\def\C{\mathbb{C}}
\def\E{\mathbb{E}}
\def\F{\mathbb{F}}
\def\H{\mathbb{H}}
\def\K{\mathbb{K}}
\def\M{\mathbb{M}}
\def\N{\mathbb{N}}
\def\P{\mathbb{P}}
\def\Q{\mathbb{Q}}
\def\R{\mathbb{R}}
\def\s{\mathbb{S}}
\def\U{\mathbb{U}}
\def\Z{\mathbb{Z}}
%
%
%% Calligraphic letters
\let\@@angstroem=\AA    
\let\angstroem=\@@angstroem
\def\AA{\mathcal{A}}
\def\BB{\mathcal{B}}
\def\CC{\mathcal{C}}
\def\DD{\mathcal{D}}
\def\EE{\mathcal{E}}
\def\FF{\mathcal{F}}
\def\GG{\mathcal{G}}
\def\HH{\mathcal{H}}
\def\II{\mathcal{I}}
\def\JJ{\mathcal{J}}
\def\KK{\mathcal{K}}
\def\LL{\mathcal{L}}
\def\MM{\mathcal{M}}
\def\NN{\mathcal{N}}
\def\OO{\mathcal{O}}
\def\PP{\mathcal{P}}
\def\QQ{\mathcal{Q}}
\def\RR{\mathcal{R}}
\def\SS{\mathcal{S}}
\def\TT{\mathcal{T}}
\def\UU{\mathcal{U}}
\def\VV{\mathcal{V}}
\def\WW{\mathcal{W}}
\def\XX{\mathcal{X}}
\def\YY{\mathcal{Y}}
\def\ZZ{\mathcal{Z}}
%
%% Morphisms
%
\newcommand{\mono}{\rightarrowtail}
\newcommand{\incl}{\hookrightarrow}
\newcommand{\epi}{\twoheadrightarrow}
\newcommand{\iso}{\stackrel{\sim}{\longrightarrow}}
\newcommand{\isoinv}{\stackrel{\sim}{\longleftarrow}}

% useful abbreviations (see LaTeX Companion, page 80)
%
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\cf}{cf.\@\xspace}

%  Various commands
\newcommand{\act}[1]{\,^{#1}}
%
%% Initialisation
\parindent.5cm\parskip0pt
%
\makeatother
\endinput
